How Novice Programmers Use and Experience ChatGPT when Solving Programming Exercises in an Introductory Course

This research paper contributes to the computing education research community's understanding of Generative AI (GenAI) in the context of introductory programming, and specifically, how students utilize related tools, such as ChatGPT. An increased understanding of students' use is mandatory for educators and higher education institutions, as GenAI is here to stay, and its performance is likely to improve rapidly in the near future. Learning about students' use patterns is not only crucial to support their learning, but to develop adequate forms of instruction and assessment. With the rapid advancement of AI, its broad availability, and ubiquitous presence in educational environments, elaborating how AI can enhance learning experiences, especially in courses such as introductory programming is important. To date, most studies have focused on the educator's perspective on GenAI, its performance, characteristics, and limitations. However, the student perspective, and how they actually use GenAI tools in course contexts, has not been subject to a great number of studies. Therefore, this study is guided by the following research questions: (1) What do students report on their use pattern of ChatGPT in the context of introductory programming exercises? and (2) How do students perceive ChatGPT in the context of introductory programming exercises? To address these questions, computing students at a large German university were asked to solve programming tasks with the assistance of ChatGPT as part of their introductory programming course. Students (n=298) provided information regarding the use of ChatGPT, and their evaluation of the tool via an online survey. This research provides a comprehensive evaluation of ChatGPT-3.5's application by novice programmers in a higher education context...

==> tables/coding-table.tex <==
\begin{table*}[htb]
\centering
\caption{How ChatGPT responds to student input (RQ1). For legend see Table~\ref{tab:legend}}
\label{tab:coding1}
\setlength{\tabcolsep}{0.2em}
%\sffamily\tiny

\begin{tabular}{
  l | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c}  %|| *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} | *{3}{c} %| *{3}{c} 
}
\hline
\multicolumn{1}{ c |}{} &
\multicolumn{18}{c|}{\scriptsize CONTENT} &
\multicolumn{9}{c|}{\scriptsize QUALITY} &
\multicolumn{6}{c}{\scriptsize OTHER}  \\
%\multicolumn{15}{c}{\scriptsize FEEDBACK TYPE}
\hline 

\multicolumn{1}{ c |}{} &
\multicolumn{3}{c|}{\textbf{INFO}} &
\multicolumn{3}{c|}{\textbf{STYLE}} & 
\multicolumn{3}{c|}{\textbf{CAUSE}}& 
\multicolumn{3}{c|}{\textbf{FIX}} &
\multicolumn{3}{c|}{\textbf{CODE}} &
\multicolumn{3}{c|}{\textbf{EXA}} &

\multicolumn{3}{c|}{\textbf{COMP}} &
\multicolumn{3}{c|}{\textbf{MIS}} &
\multicolumn{3}{c|}{\textbf{UNC}} &

\multicolumn{3}{c|}{\textbf{META}} &
\multicolumn{3}{c}{\textbf{MOT}} %&

%\multicolumn{3}{c|}{\textbf{KTC}} & 
%\multicolumn{3}{c|}{\textbf{KC}}& 
%\multicolumn{3}{c|}{\textbf{KM}} &
%\multicolumn{3}{c|}{\textbf{KH}} &
%\multicolumn{3}{c}{\textbf{KMC}}
\\
\hline %[1.5em]

\textbf{Stud\_task}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}
    & \tiny{R1} & \tiny{R2} & \tiny{R3}

%    & \tiny{R1} & \tiny{R2} & \tiny{R3}
%    & \tiny{R1} & \tiny{R2} & \tiny{R3}
%    & \tiny{R1} & \tiny{R2} & \tiny{R3}
%    & \tiny{R1} & \tiny{R2} & \tiny{R3}
%    & \tiny{R1} & \tiny{R2} & \tiny{R3}
     \\ %[0.2cm]
    
    %\textbf{Name} & \textbf{Practice type} & %\textbf{Feedback types} & \textbf{Feedback %timing} & \textbf{Feedback presentation?} 

\hline

\student{01\_TEOS} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \noSym & \yesSym & \yesSym        %Explanation Cause of Error
& \noSym & \noSym & \noSym         %Explanation Fix of Error
& \yesSym & \partSym & \yesSym      %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & -- & \yesSym            %Compilable
& \noSym & \yesSym & \yesSym        %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{02\_TEOS}  
& \noSym & \noSym & \noSym          %Requesting Information
& \yesSym & \yesSym & \yesSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & \yesSym & \yesSym       %Compilable
& \yesSym & \yesSym & \noSym        %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{03\_TEOS} 
& \noSym & \yesSym & \noSym         %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \partSym & \noSym & \noSym        %Code Provided
& \noSym & \noSym & \noSym        %Examples
& -- & -- & --                      %Compilable
& \yesSym & \noSym & \noSym         %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{04\_TEOS} 
& \noSym & \noSym & \noSym         %Requesting Information
& \noSym & \yesSym & \noSym         %Stylistic Suggestion
& \noSym & \noSym & \noSym         %Explanation Cause of Error
& \noSym & \noSym & \noSym         %Explanation Fix of Error
& \noSym & \noSym & \noSym          %Code Provided
& \noSym & \noSym & \noSym          %Examples
& -- & -- & --                      %Compilable
& \noSym & \noSym & \noSym          %Misleading Information
& \yesSym & \yesSym & \yesSym       %Uncertainty
& \yesSym & \yesSym & \yesSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{05\_TEOS}
& \noSym & \noSym & \noSym          %Requesting Information
& \yesSym & \yesSym & \yesSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & \yesSym & \yesSym       %Compilable
& \noSym & \noSym & \noSym          %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{06\_TEOS}
& \noSym & \noSym & \noSym          %Requesting Information
& \yesSym & \noSym & \yesSym        %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \partSym & \yesSym & \partSym     %Code Provided
& \yesSym & \yesSym & \yesSym       %Examples
& -- & \yesSym & --                 %Compilable
& \noSym & \noSym & \noSym          %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{07\_TEOS} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \noSym        %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & \yesSym & --            %Compilable
& \noSym & \yesSym & \noSym         %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{08\_TEOS}
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \yesSym & \noSym         %Stylistic Suggestion
& \yesSym & \noSym & \yesSym        %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \partSym & \noSym & \noSym        %Code Provided
& \noSym & \noSym & \noSym          %Examples
& -- & -- & --                      %Compilable
& \noSym & \noSym & \noSym          %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \yesSym & \noSym & \noSym        %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{09\_TEOS} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \yesSym & \noSym         %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & \yesSym & \yesSym       %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{10\_TEOS} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \yesSym & \noSym         %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \noSym & \yesSym & \yesSym        %Compilable
& \yesSym & \noSym & \noSym         %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC



%%%%%%%%%%%%%%%%%%
%%%%%  HIEKE %%%%%
%%%%%%%%%%%%%%%%%%

\\
%\hline
\student{01\_TTBS} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \noSym & \yesSym & \yesSym       %Explanation Fix of Error
& \noSym & \yesSym & \yesSym        %Code Provided
& \noSym & \yesSym & \noSym         %Examples
& -- & \yesSym & \yesSym                %Compilable
& \yesSym & \noSym & \noSym          %Misleading Information
& \yesSym & \noSym & \noSym         %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{02\_TTBS} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym      %Code Provided
& \noSym & \noSym & \yesSym         %Examples
& -- & \yesSym & \yesSym            %Compilable
& \noSym & \noSym & \noSym       %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{03\_TTBS} 
& \noSym & \noSym & \yesSym         %Requesting Information
& \noSym & \yesSym & \yesSym        %Stylistic Suggestion
& \yesSym & \noSym & \yesSym       %Explanation Cause of Error
& \yesSym & \noSym & \noSym         %Explanation Fix of Error
& \yesSym & \noSym & \noSym         %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & -- & --                %Compilable
& \yesSym & \noSym & \yesSym        %Misleading Information
& \noSym & \noSym & \yesSym         %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{04\_TTBS} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \partSym & \yesSym      %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & \yesSym & --                %Compilable
& \noSym & \noSym & \yesSym          %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{05\_TTBA} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \yesSym         %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \partSym & \yesSym & \yesSym      %Code Provided
& \noSym & \yesSym & \noSym          %Examples
& -- & \yesSym & \yesSym                %Compilable
& \noSym & \yesSym & \yesSym        %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{06\_TTBA} 
    & \noSym & \noSym & \noSym      %Requesting Information
& \yesSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym        %Explanation Fix of Error
& \noSym & \yesSym & \partSym       %Code Provided
& \noSym & \noSym & \noSym          %Examples
& -- & \yesSym & --                %Compilable
& \yesSym & \yesSym & \yesSym          %Misleading Information
& \yesSym & \noSym & \noSym         %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{07\_TTBA} 
& \noSym & \noSym & \noSym          %Requesting Information
& \yesSym & \yesSym & \noSym        %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \noSym & \partSym & \partSym        %Code Provided
& \noSym & \noSym & \yesSym         %Examples
& -- & -- & --                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \yesSym & \noSym         %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{08\_TTBA} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \yesSym & \noSym & \yesSym        %Examples
& \yesSym & \noSym & \yesSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{09\_TTBA} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \noSym & \yesSym        %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym          %Examples
& \yesSym & \yesSym & \yesSym                %Compilable
& \yesSym & \noSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{10\_TTBA} 
& \noSym & \noSym & \noSym          %Requesting Information
& \noSym & \noSym & \noSym          %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym        %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \yesSym & \noSym & \noSym         %Examples
& \yesSym & \yesSym & \yesSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym          %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym          %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
%%%%%%%%%%%%%%%%%%%%%%
%% Natalie %%%%%%%%%%%

\\
%\hline
\student{01\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \noSym & \yesSym & \yesSym       %Stylistic Suggestion
& \yesSym & \noSym & \yesSym       %Explanation Cause of Error
& \yesSym & \noSym & \yesSym       %Explanation Fix of Error
& \yesSym & \noSym & \noSym       %Code Provided
& \yesSym & \noSym & \noSym       %Examples
& \yesSym & -- & --                %Compilable
& \yesSym & \noSym & \yesSym       %Misleading Information
& \noSym & \yesSym & \yesSym       %Uncertainty
& \noSym & \yesSym & \noSym       %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{02\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \noSym & \noSym & \yesSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \noSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& \yesSym & \yesSym & --         %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \yesSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \yesSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{03\_NEGF} 
& \noSym & \noSym & \noSym       %Requesting Information
& \noSym & \noSym & \yesSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& \yesSym & \yesSym & \yesSym       %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \yesSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{04\_NEGF}
& \yesSym & \noSym & \noSym       %Requesting Information
& \noSym & \noSym & \yesSym       %Stylistic Suggestion
& \yesSym & \yesSym & \noSym       %Explanation Cause of Error
& \noSym & \yesSym & \noSym       %Explanation Fix of Error
& \noSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& -- & \yesSym & \yesSym                %Compilable
& \noSym & \yesSym & \yesSym       %Misleading Information
& \yesSym & \noSym & \yesSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{05\_NEGF}
& \noSym & \yesSym & \noSym       %Requesting Information
& \noSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \noSym & \noSym       %Explanation Cause of Error
& \yesSym & \noSym & \noSym       %Explanation Fix of Error
& \partSym & \noSym & \noSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& -- & -- & --                %Compilable
& \noSym & \noSym & \noSym       %Misleading Information
& \yesSym & \yesSym & \yesSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{06\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \yesSym & \yesSym & \yesSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \noSym & \yesSym       %Explanation Fix of Error
& \yesSym & \noSym & \noSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& \yesSym & -- & --                %Compilable
& \yesSym & \noSym & \noSym       %Misleading Information
& \yesSym & \yesSym & \yesSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{07\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \noSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \partSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& -- & -- & \yesSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{08\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \yesSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& \yesSym & -- & \yesSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym       %Uncertainty
& \noSym & \noSym & \noSym       %Metacognitive
& \yesSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{09\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \yesSym & \yesSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \yesSym       %Examples
& \noSym & \noSym & \noSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{10\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \yesSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& \yesSym & \yesSym & \yesSym                %Compilable
& \yesSym & \noSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym       %Uncertainty
& \noSym & \noSym & \noSym       %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{11\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \noSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \noSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& \noSym & \noSym & \yesSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \noSym & \noSym       %Uncertainty
& \noSym & \noSym & \noSym       %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{12\_NEGF} 
& \noSym & \noSym & \noSym       %Requesting Information
& \noSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \yesSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& \yesSym & \yesSym & \yesSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \yesSym & \noSym & \noSym       %Uncertainty
& \noSym & \noSym & \noSym          %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\
\student{13\_NEGF}
& \noSym & \noSym & \noSym       %Requesting Information
& \noSym & \noSym & \noSym       %Stylistic Suggestion
& \yesSym & \yesSym & \yesSym       %Explanation Cause of Error
& \yesSym & \yesSym & \yesSym       %Explanation Fix of Error
& \partSym & \yesSym & \yesSym       %Code Provided
& \noSym & \noSym & \noSym       %Examples
& -- & \yesSym & \noSym                %Compilable
& \yesSym & \yesSym & \yesSym       %Misleading Information
& \noSym & \yesSym & \yesSym       %Uncertainty
& \noSym & \noSym & \noSym       %Metacognitive
& \noSym & \noSym & \noSym       %Motivation

%& \noSym & \noSym & \noSym          %KTC
%& \noSym & \noSym & \noSym          %KC
%& \noSym & \noSym & \noSym          %KM
%& \noSym & \noSym & \noSym          %KH
%& \noSym & \noSym & \noSym          %KMC
\\

%\multicolumn{31}{c}{\yesSym: Yes \quad \noSym: No \quad \partSym: Partial}
\multicolumn{31}{c}{\yesSym: Yes \quad \noSym: No \quad \partSym: Snippet \quad --: Not applicable}
%\hline

\end{tabular}

%\vspace{8px}
\end{table*}

==> tables/table_categories.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% METICULOUS disposition %%%%%%%%%%%%%%%%%
 % \begin{comment}
\begin{table*}[t!]
\centering \scriptsize
\caption{Coding scheme with categories, definitions, and anchor examples for students' perception of ChatGPT. 
%\caption{\textit{Meticulous} coding scheme with categories, definitions, and anchor examples}
\label{tab:categories}
\resizebox{\linewidth}{!}{ % start resizing 
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Category} & \textbf{Definition} & \textbf{Anchor Example(s)} \\ \midrule 
\multirow{2}{*}{\makecell[l]{Paying close\\ attention to detail}} 
    & \makecell[l]{Comprising the details to which students direct their attention, \\
                  e.g., formatting, comments, correct syntax, visualizations, spelling \\ 
                  alignment, brackets, linting errors, readability, checking dependencies}
    & \multirow{2}{*}{\makecell[l]{\say{I went through the entire program looking at every single line of code to make\\sure everything was written properly} \\ 
                \say{We rechecked multiple times that all relationship types in the graph were correct.}}
    } \\ \cline{2-2}
    & \makecell[l]{Conducting repetitive checks of a solution\vspace{0.5em}} & \\ \hline

\makecell[l]{Producing the\\correct solution} 
    & \makecell[l]{Stresses the actions required to achieve a correct solution\\to the task and its requirements.} 
    & \makecell[l]{
                \say{I made sure I followed every direction in the rubric and did not cut any corners.\\
                I used everything I was instructed to use in the program and made sure it\\
                functioned properly}} \\ \hline

\makecell[l]{Improving solution\\(even if not required)} 
    & \makecell[l]{Highlighting intrinsically motivated work, although not requested by\\
                the task description, e.g., to make the solution more legible for other\\
                programmers, or to improve its quality (e.g., runtime, accuracy,\\
                reducing lines of code, etc.)\vspace{0.5em}} 
    & \makecell[l]{
            \say{I was always looking for ways to improve my program to make it easier to read\\and understand by any future programmers}\\
            \say{I remember using some code that wasn't necessarily required for the assignment.}} \\ \hline


\makecell[l]{Testing code\\thoroughly} 
    & \makecell[l]{Testing code to ensure it functions in different cases by using test\\
                    scripts, test data, and addressing the occurring exceptions and errors.} 
    & \makecell[l]{
        \say{I checked each query result multiple times to make sure that I was 
        completely\\
        satisfied with how specific the results were. We also made sure
        that there was\\enough data to make sure every query looked good too.}\\
        \say{[...] I made sure there were neither errors nor warnings when I ran the test script.}} \\ \hline

\makecell[l]{Accepting \\feedback} 
    & \makecell[l]{Recognition of feedback from collaborators or educators with the goal\\
                of implementing it and improving the solution.} 
    & \makecell[l]{
                \say{We always tried to take the feedback and accurately modify our work so that it\\
                would meet the requirements of the project}} \\ \hline

\makecell[l]{Applying time man-\\agement strategies for\\a timely submission} 
    & \makecell[l]{Planning to conduct the work ahead of time to not run out of time\\
                before completing the assignment.} 
    & \makecell[l]{
                \say{I will always get an assignment/work done ahead of time because I hate the\\
                burden of it on my shoulders throughout the week.}} \\ \bottomrule
\end{tabular}
} % end resizing
\end{table*}
